Precision Physics with Muons : A Decade of Theoretical and Experimental Advances

The muon has been instrumental in establishing the Standard Model of particle physics and continues to play a key role in exploring the nature of New Physics. A global program is underway to enhance the discovery potential of a wide range of muon probes, with significant increases in sensitivity anticipated over the next decade. In this review, we examine recent experimental advancements in the study of muon decays, the determination of the muon magnetic and electric dipole moments, and the search for charged lepton flavor-violating transitions. We explore the implications for scenarios of physics beyond the Standard Model, focusing on models involving light new particles, such as axions and hidden sectors. Opportunities from novel experimental concepts and proposal for new muon facilities are also discussed.

==> symbols.tex <==
\RequirePackage{xspace}

%   text mode macros
\def\ie{{\it i.e.}}
\def\eg{{\it e.g.}}
\def\etc{{\it etc.}}
\def\etal{{\it et al.}}
\def\ibid{{\it ibid}.}

%  equation display macros
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}

\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em B\kern-0.1em{\smaller
A\kern-0.2em R}}}


%%  multiple-line equations  (use \CR as the carriage return):
\newenvironment{Eqnarray}%
   {\arraycolsep 0.14em\begin{eqnarray}}{\end{eqnarray}}
\def\beqa{\begin{Eqnarray}}
\def\eeqa#1{\label{#1}\end{Eqnarray}}
\def\eeqan{\end{Eqnarray}}
\def\CR{\nonumber \\ }

\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}

\newcommand{\mmbar}{M_\mu-\overline{M}_\mu}
\newcommand{\mmu}{{M_\mu}}
\newcommand{\mmup}{{M_\mu^P}}
\newcommand{\mmuv}{{M_\mu^V}}
\newcommand{\ammu}{{\overline{M}_\mu}}
\newcommand{\ammup}{{\bar{M}_\mu^P}}
\newcommand{\ammuv}{{\bar{M}_\mu^V}}

\def\CPc               {\ensuremath{C\!Pc}\xspace}
\def\CPv               {\ensuremath{C\!Pv}\xspace}
\def\CP                {\ensuremath{C\!P}\xspace}
\def\CPT               {\ensuremath{C\!PT}\xspace} % Looks better without \!



%%  reference to an equation number:
\def\leqn#1{(\ref{#1})}

%%  sizing and bars
\def\st{\scriptstyle}
\def\sst{\scriptscriptstyle}

\def\overbar#1{\overline{#1}}
\let\littlebar=\bar
\let\bar=\overbar

\def\subscr#1{{\mbox{\scriptsize #1}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  expectation values: 

\def\VEV#1{\left\langle{ #1} \right\rangle}
\def\bra#1{\left\langle{ #1} \right|}
\def\ket#1{\left| {#1} \right\rangle}
\def\vev#1{\langle #1 \rangle}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% relation symbols

\def\lsim{\mathrel{\raise.3ex\hbox{$<$\kern-.75em\lower1ex\hbox{$\sim$}}}}
\def\gsim{\mathrel{\raise.3ex\hbox{$>$\kern-.75em\lower1ex\hbox{$\sim$}}}}

\def\Im{{\rm Im}}
\def\Re{{\rm Re}}
\def\tr{{ \rm tr}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  caligraphic letters (for matrix elements, luminosity, etc.)

\def\D{{\cal D}}
\def\L{{\cal L}}
\def\M{{\cal M}}
\def\O{{\cal O}}
\def\W{{\cal W}}
\def\H{{\cal H}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  matrix operations and fractions:

\def\One{{\bf 1}}
\def\hc{{\mbox{\rm h.c.}}}
\def\tr{{\mbox{\rm tr}}}
\def\half{\frac{1}{2}}
\def\thalf{\frac{3}{2}}
\def\third{\frac{1}{3}}
\def\tthird{\frac{2}{3}}

\def\del{\partial}
\def\Dslash{\not{\hbox{\kern-4pt $D$}}}
\def\dslash{\not{\hbox{\kern-2pt $\del$}}}
\def\pslash{\not{\hbox{\kern-2pt $p$}}}
\def\ETmiss{\not{\hbox{\kern-4pt $E$}}_T}

\def\Dlr{\mathrel{\raise1.5ex\hbox{$\leftrightarrow$\kern-1em\lower1.5ex\hbox{$D$}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  high-energy physics terminology:

\def\Pl{{\mbox{\scriptsize Pl}}}
\def\eff{{\mbox{\scriptsize eff}}}
\def\CM{{\mbox{\scriptsize CM}}}
\def\GUT{{\mbox{\scriptsize GUT}}}
\def\BR{\mbox{\rm BR}}
\def\ee{e^+e^-}
\def\sstw{\sin^2\theta_w}
\def\cstw{\cos^2\theta_w}
\def\mz{m_Z}
\def\gz{\Gamma_Z}
\def\mw{m_W}
\def\gw{\Gamma_W}
\def\mt{m_t}
\def\gt{\Gamma_t}
\def\mh{m_H}
\def\gh{\Gamma_H}
\def\gmu{G_\mu}
\def\GF{G_F}
\def\alphas{\alpha_s}
\def\MSB{{\bar{M \kern -2pt S}}}
\def\msb{{\bar{\scriptsize M \kern -1pt S}}}
\def\lmsb{\Lambda_{\msb}}
\def\drb{{\bar{\scriptsize D \kern -1pt R}}}
\def\ELER{e^-_Le^+_R}
\def\EREL{e^-_Re^+_L}
\def\ELEL{e^-_Le^+_L}
\def\ERER{e^-_Re^+_R}
\def\eps{\epsilon}
\def\Kzero{K^0}
\def\Kzerobar{{\bar K}^0}
\def\Dzero{D^0}
\def\Dzerobar{{\bar D}^0}
\def\Bzero{B^0}
\def\Bzerobar{{\bar B}^0}


%%%%%%%%%%%%   units for math mode  %%%%%%%%%%%%%%%%%%%%%%%%%

\def\ifb{{\rm fb}^{-1}}
\def\eV{{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}}
\def\keV{{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}}
\def\MeV{{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}}
\def\GeV{{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}}
\def\TeV{{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}}
\def\keVc{{\ensuremath{\mathrm{\,ke\kern -0.1em V/c}}\xspace}}
\def\MeVc{{\ensuremath{\mathrm{\,Me\kern -0.1em V/c}}\xspace}}
\def\GeVc{{\ensuremath{\mathrm{\,Ge\kern -0.1em V/c}}\xspace}}
\def\TeVc{{\ensuremath{\mathrm{\,Ge\kern -0.1em V/c}}\xspace}}
\def\keVcc{{\ensuremath{\mathrm{\,ke\kern -0.1em V/c^2}}\xspace}}
\def\MeVcc{{\ensuremath{\mathrm{\,Me\kern -0.1em V/c^2}}\xspace}}
\def\GeVcc{{\ensuremath{\mathrm{\,Ge\kern -0.1em V/c^2}}\xspace}}
\def\TeVcc{{\ensuremath{\mathrm{\,Te\kern -0.1em V/c^2}}\xspace}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  supersymmetry:

\def\ch#1{\widetilde\chi^+_{#1}}
\def\chm#1{\widetilde\chi^-_{#1}}
\def\neu#1{\widetilde\chi^0_{#1}}
\def\s#1{\widetilde{#1}}




